End-to-End Video Question Answering with Frame Scoring Mechanisms and Adaptive Sampling

Video Question Answering (VideoQA) has emerged as a challenging frontier in the field of multimedia processing, requiring intricate interactions between visual and textual modalities. Simply uniformly sampling frames or indiscriminately aggregating frame-level visual features often falls short in capturing the nuanced and relevant contexts of videos to well perform VideoQA. To mitigate these issues, we propose VidF4, a novel VideoQA framework equipped with tailored frame selection strategy for effective and efficient VideoQA. We propose three frame-scoring mechanisms that consider both question relevance and inter-frame similarity to evaluate the importance of each frame for a given question on the video. Furthermore, we design a differentiable adaptive frame sampling mechanism to facilitate end-to-end training for the frame selector and answer generator. The experimental results across three widely adopted benchmarks demonstrate that our model consistently outperforms existing VideoQA methods, establishing a new SOTA across NExT-QA (+0.3%), STAR (+0.9%), and TVQA (+1.0%). Furthermore, through both quantitative and qualitative analyses, we validate the effectiveness of each design choice.

==> 1_figures/efficiency.tex <==
% \begin{figure}[!tb]
%     \centering
%     \includegraphics[scale=0.52]{0_pictures/efficiency1.pdf}
%     \caption{Comparison of model performance on STAR with different numbers of frames used during inference, where the same color represents the same model. Dashed line denotes the testing performance when using the same number of frames as like training.}
%     \label{fig:topK_frame}
% \end{figure}

\begin{figure*}

  \begin{minipage}[t]{0.48\linewidth} % 如果一行放2个图，用0.5，如果3个图，用0.33
    \centering 
    \subfigure b{
    % \label{fig:cr2c}
    \includegraphics[width=1.0\textwidth]{0_pictures/efficiency.pdf}}
    
  \end{minipage}%
    \begin{minipage}[t]{0.25\linewidth} 
    \centering 
    \subfigure a{
    
    \includegraphics[width=1.0\textwidth]{0_pictures/flops.pdf}}
  \end{minipage} 
  % \begin{minipage}[t]{0.32\linewidth} 
  %   \centering 
  %   \subfigure c{
  %   \label{fig:r2c}
  %   \includegraphics[width=1.0\textwidth]{0_pictures/efficiency.pdf}}
    
  % \end{minipage} 
  \caption{(a) Comparison of model performance on STAR with different numbers of frames used during inference, where the same color represents the same model. Dashed line denotes the testing performance when using the same number of frames as like training.}

\label{fig:topK_frame}
\end{figure*}

==> 1_figures/overall_arch.tex <==
% \begin{figure*}[!thb]
%     \centering
%     \includesvg[scale=0.15]{pic/v2-1.svg}
%     \caption{arch. v1}
% \end{figure*}

\begin{figure*}[!thb]
    \centering
    \includegraphics[scale=0.12]{0_pictures/v3-2.png}
    \caption{2nd version: size, legend arrows,}
    \label{fig:overall framework}
\end{figure*}

==> 2_tables/inference.tex <==
\begin{table}[!hbt]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{\#Frames} & 
\multicolumn{5}{c}{\textbf{STAR}} \\
&\textbf{Int.}  &\textbf{Seq.}  &\textbf{Pre.}  &\textbf{Fea.}  &\textbf{Tot.}  \\ 
 \midrule
 
 % \multicolumn{6}{c}{Training} \\
 % \midrule
% \rowcolor{gray!5}32$\xrightarrow{}$4 &62.3  &64.7  &57.4  &54.9  &62.6    \\
% \midrule
% \multicolumn{6}{c}{Inference } \\
% \midrule

\rowcolor{gray!10}32$\xrightarrow{}$8 &68.4  &70.4  &60.9  &59.4  &68.1    \\
\rowcolor{gray!20}32$\xrightarrow{}$16 &69.3  &71.7  &63.6  &59.8  &69.3   \\
% 32$\xrightarrow{}$12 &-    &    \\
% 32$\xrightarrow{}$14 &-    &    \\
\rowcolor{gray!30}32$\xrightarrow{}$32 &69.6  &72.8  &64.3  &62.0  &70.2    \\

\midrule


\end{tabular}
}
\caption{During the training, 8 frames are selected from 32 frames. In the inference, select 8 frames, 16 frames, or all 32 frames.}
% - indicates the non-use of that component.} 
\label{tb: inference}
%
% \vspace{-3mm}
\end{table}




==> 3_sections/6_Limitations.tex <==



\section*{Limitations}

As elaborated in this paper, we aim to highlight the role of frame selection in VideoQA, which is also the main focus of this paper. However, the alignment and understanding of visual information and text by the answer generator are equally crucial, and this will be a key topic of investigation in our future work.


